Amplitude-Based Sequential Optimization of Energy Harvesting with Reconfigurable Intelligent Surfaces

Reconfigurable Intelligent Surfaces (RISs) have gained immense popularity in recent years because of their ability to improve wireless coverage and their flexibility to adapt to the changes in a wireless environment. These advantages are due to RISs' ability to control and manipulate radio frequency (RF) wave propagation. RISs may be deployed in inaccessible locations where it is difficult or expensive to connect to the power grid. Energy harvesting can enable the RIS to self-sustain its operations without relying on external power sources. In this paper, we consider the problem of energy harvesting for RISs in the absence of coordination with the ambient RF source. We consider both direct and indirect energy harvesting scenarios and show that the same mathematical model applies to them. We propose a sequential phase-alignment algorithm that maximizes the received power based on only power measurements. We prove the convergence of the proposed algorithm to the optimal value under specific circumstances. Our simulation results show that the proposed algorithm converges to the optimal solution in a few iterations and outperforms the random phase update method in terms of the number of required measurements.

==> Unused_Figures/Indirect_RIS.tex <==
% \definecolor{azure}{rgb}{0.0, 0.5, 1.0}
% \definecolor{awesome}{rgb}{1.0, 0.13, 0.32}
% \definecolor{amber}{rgb}{1.0, 0.49, 0.0}
%\definecolor{darkpastelgreen}{rgb}{0.01, 0.75, 0.24}
\definecolor{mycolor1}{rgb}{0.85,0.325,0.098}
\definecolor{mycolor2}{rgb}{0.00000,0.44700,0.74100}
\definecolor{mycolor3}{rgb}{0.00000,0.49804,0.00000}

\definecolor{apricot}{rgb}{0.98, 0.81, 0.69}
\definecolor{copper}{rgb}{0.72, 0.45, 0.2}
\definecolor{babyblue}{rgb}{0.54, 0.81, 0.94}
\definecolor{gray}{rgb}{0.5, 0.5, 0.5}
\usetikzlibrary{decorations.pathreplacing}

\begin{tikzpicture}[cross/.style={path picture={ 
  \draw[black]
(path picture bounding box.south east) -- (path picture bounding box.north west) (path picture bounding box.south west) -- (path picture bounding box.north east);
}}]
\pgfmathsetmacro{\R}{1}
\pgfmathsetmacro{\W}{0.8}
\pgfmathsetmacro{\H}{0.6}
%\tikzstyle{every node}=[trapezium, draw, minimum width=\R cm, minimum height=\R,
%trapezium left angle=60, trapezium right angle=120]

\foreach \i in {-4,...,3} {
    \foreach \j in {-4,...,3} {
    \node [draw, copper, very thick,trapezium, trapezium left angle=60, trapezium right angle=120, minimum width=\R cm,outer sep=0pt,fill=none, rotate = 30] at (\i*\W*cos{30},\i*\W*sin{30}+\j*\H) {};
    \draw[dashed, mycolor3] (\i*\W*cos{30},\i*\W*sin{30}+\j*\H) -- (6,2);
    \draw[copper,very thick] (\i*\W*cos{30},\i*\W*sin{30}+\j*\H-0.46*\H) -- (\i*\W*cos{30},\i*\W*sin{30}+\j*\H-0.1*\H);
    \draw[copper,very thick] (\i*\W*cos{30},\i*\W*sin{30}+\j*\H+0.46*\H) -- (\i*\W*cos{30},\i*\W*sin{30}+\j*\H+0.1*\H);
    \draw[copper,very thick] (\i*\W*cos{30}-0.1*\W,\i*\W*sin{30}+\j*\H-0.1*\H-0.1*\W*sin{30}) -- (\i*\W*cos{30}+0.1*\W,\i*\W*sin{30}+\j*\H-0.1*\H+0.1*\W*sin{30});
    \draw[copper,very thick] (\i*\W*cos{30}-0.1*\W,\i*\W*sin{30}+\j*\H+0.1*\H-0.1*\W*sin{30}) -- (\i*\W*cos{30}+0.1*\W,\i*\W*sin{30}+\j*\H+0.1*\H+0.1*\W*sin{30});}}    
    \node[] at (7.4,2) {\large EH device};
    \node[mycolor2] at (8.2,0.8) {\large Near-field focusing};
    \draw[mycolor2,very thick,dotted] (6,2) ellipse (0.3 and 0.6);
    \draw[mycolor2,-stealth, thick] (6,1.4) -- (6,0.8) -- (6.5,0.8);

\draw[thick] (-3.18,-4.47) -- (-3.18,0.33)--(2.29,3.47);
\end{tikzpicture}


==> Unused_Figures/Proposed_vs_random.tex <==
\definecolor{mycolor1}{rgb}{0.85,0.325,0.098}
\definecolor{mycolor2}{rgb}{0.00000,0.44700,0.74100}
\definecolor{mycolor3}{rgb}{0.00000,0.49804,0.00000}
\pgfplotsset{major grid style = {dotted, gray}}
\pgfplotsset{minor grid style = {dotted, gray}}
\begin{tikzpicture}
\begin{axis}[%
width=0.46*6.028in,
height=0.46*4.754in,
at={(1.011in,0.642in)},
scale only axis,
xmin=0,
xmax=5000,
xlabel style={font=\color{white!15!black}},
xlabel={\small Number of measurements},
ymin=0,
ymax=1,
ylabel style={font=\color{white!15!black}, yshift=-2mm},
ylabel={\small Mean normalized achieved power},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={at={(0.99,0.01)}, anchor=south east, legend cell align=left, align=left, draw=none, inner sep=0.001pt, outer sep=0.001pt, row sep=0pt}
]
\addplot [color=mycolor2, mark repeat=1, line width=1.0pt, mark=none, mark options={mark size=2pt,solid, line width=0.5pt}]
  table[row sep=crcr]{%
0	0.0130914825812426\\
30	0.0405199106975778\\
60	0.0842848872987536\\
90	0.143056520431794\\
120	0.219471231744576\\
150	0.31217010247734\\
180	0.41901059832333\\
210	0.541353716713789\\
240	0.676625507943281\\
270	0.829447891507858\\
300	0.995319523270042\\
330	0.998023808704362\\
360	0.998817431264077\\
390	0.999204428574643\\
420	0.999444196311743\\
450	0.999615849916358\\
480	0.999733260460846\\
510	0.999815431404869\\
540	0.999886020012035\\
570	0.99993478109223\\
600	0.999968060562337\\
630	0.999981984003441\\
660	0.99998836301282\\
690	0.999992112913441\\
720	0.999994573583988\\
750	0.999996231024903\\
780	0.999997437256219\\
810	0.999998326924509\\
840	0.999998903411165\\
870	0.99999931244487\\
900	0.999999600372748\\
930	0.9999997458159\\
960	0.99999983312162\\
990	0.999999886875469\\
1020	0.999999923016472\\
1050	0.999999948886677\\
1080	0.999999966093726\\
1110	0.999999976907346\\
1140	0.999999985116657\\
1170	0.999999990753904\\
1200	0.999999994146349\\
1230	0.999999996177885\\
1260	0.999999997482207\\
1290	0.999999998324326\\
1320	0.999999998889232\\
1350	0.9999999992525\\
1380	0.999999999497964\\
1410	0.999999999674674\\
1440	0.999999999791305\\
1470	0.999999999864202\\
1500	0.999999999912045\\
1530	0.999999999943027\\
1560	0.999999999962728\\
1590	0.99999999997495\\
1620	0.999999999983128\\
1650	0.99999999998888\\
1680	0.999999999992822\\
1710	0.999999999995262\\
1740	0.99999999999686\\
1770	0.999999999997973\\
1800	0.999999999998702\\
1830	0.999999999999142\\
1860	0.99999999999943\\
1890	0.999999999999622\\
1920	0.999999999999753\\
1950	0.99999999999984\\
1980	0.999999999999894\\
2010	0.999999999999933\\
2040	0.99999999999996\\
2070	0.999999999999978\\
2100	0.999999999999988\\
2130	0.999999999999994\\
2160	0.999999999999997\\
2190	0.999999999999999\\
2220	0.999999999999999\\
2250	1\\
2280	1\\
2310	1\\
2340	1\\
2370	1\\
2400	1\\
2430	1\\
2460	1\\
2490	1\\
2520	1\\
2550	1\\
2580	1\\
2610	1\\
2640	1\\
2670	1\\
2700	1\\
2730	1\\
2760	1\\
2790	1\\
2820	1\\
2850	1\\
2880	1\\
2910	1\\
2940	1\\
2970	1\\
3000	1\\
3030	1\\
3060	1\\
3090	1\\
3120	1\\
3150	1\\
3180	1\\
3210	1\\
3240	1\\
3270	1\\
3300	1\\
3330	1\\
3360	1\\
3390	1\\
3420	1\\
3450	1\\
3480	1\\
3510	1\\
3540	1\\
3570	1\\
3600	1\\
3630	1\\
3660	1\\
3690	1\\
3720	1\\
3750	1\\
3780	1\\
3810	1\\
3840	1\\
3870	1\\
3900	1\\
3930	1\\
3960	1\\
3990	1\\
4020	1\\
4050	1\\
4080	1\\
4110	1\\
4140	1\\
4170	1\\
4200	1\\
4230	1\\
4260	1\\
4290	1\\
4320	1\\
4350	1\\
4380	1\\
4410	1\\
4440	1\\
4470	1\\
4500	1\\
4530	1\\
4560	1\\
4590	1\\
4620	1\\
4650	1\\
4680	1\\
4710	1\\
4740	1\\
4770	1\\
4800	1\\
4830	1\\
4860	1\\
4890	1\\
4920	1\\
4950	1\\
4980	1\\
5010	1\\
5040	1\\
5070	1\\
5100	1\\
5130	1\\
5160	1\\
5190	1\\
5220	1\\
5250	1\\
5280	1\\
5310	1\\
5340	1\\
5370	1\\
5400	1\\
5430	1\\
5460	1\\
5490	1\\
5520	1\\
5550	1\\
5580	1\\
5610	1\\
5640	1\\
5670	1\\
5700	1\\
5730	1\\
5760	1\\
5790	1\\
5820	1\\
5850	1\\
5880	1\\
5910	1\\
5940	1\\
5970	1\\
6000	1\\
6030	1\\
6060	1\\
6090	1\\
6120	1\\
6150	1\\
6180	1\\
6210	1\\
6240	1\\
6270	1\\
6300	1\\
6330	1\\
6360	1\\
6390	1\\
6420	1\\
6450	1\\
6480	1\\
6510	1\\
6540	1\\
6570	1\\
6600	1\\
6630	1\\
6660	1\\
6690	1\\
6720	1\\
6750	1\\
6780	1\\
6810	1\\
6840	1\\
6870	1\\
6900	1\\
6930	1\\
6960	1\\
6990	1\\
7020	1\\
7050	1\\
7080	1\\
7110	1\\
7140	1\\
7170	1\\
7200	1\\
7230	1\\
7260	1\\
7290	1\\
7320	1\\
7350	1\\
7380	1\\
7410	1\\
7440	1\\
7470	1\\
7500	1\\
7530	1\\
7560	1\\
7590	1\\
7620	1\\
7650	1\\
7680	1\\
7710	1\\
7740	1\\
7770	1\\
7800	1\\
7830	1\\
7860	1\\
7890	1\\
7920	1\\
7950	1\\
7980	1\\
8010	1\\
8040	1\\
8070	1\\
8100	1\\
8130	1\\
8160	1\\
8190	1\\
8220	1\\
8250	1\\
8280	1\\
8310	1\\
8340	1\\
8370	1\\
8400	1\\
8430	1\\
8460	1\\
8490	1\\
8520	1\\
8550	1\\
8580	1\\
8610	1\\
8640	1\\
8670	1\\
8700	1\\
8730	1\\
8760	1\\
8790	1\\
8820	1\\
8850	1\\
8880	1\\
8910	1\\
8940	1\\
8970	1\\
9000	1\\
9030	1\\
9060	1\\
9090	1\\
9120	1\\
9150	1\\
9180	1\\
9210	1\\
9240	1\\
9270	1\\
9300	1\\
9330	1\\
9360	1\\
9390	1\\
9420	1\\
9450	1\\
9480	1\\
9510	1\\
9540	1\\
9570	1\\
9600	1\\
9630	1\\
9660	1\\
9690	1\\
9720	1\\
9750	1\\
9780	1\\
9810	1\\
9840	1\\
9870	1\\
9900	1\\
9930	1\\
9960	1\\
9990	1\\
10020	1\\
10050	1\\
10080	1\\
10110	1\\
10140	1\\
10170	1\\
10200	1\\
10230	1\\
10260	1\\
10290	1\\
10320	1\\
10350	1\\
10380	1\\
10410	1\\
10440	1\\
10470	1\\
10500	1\\
10530	1\\
10560	1\\
10590	1\\
10620	1\\
10650	1\\
10680	1\\
10710	1\\
10740	1\\
10770	1\\
10800	1\\
10830	1\\
10860	1\\
10890	1\\
10920	1\\
10950	1\\
10980	1\\
11010	1\\
11040	1\\
11070	1\\
11100	1\\
11130	1\\
11160	1\\
11190	1\\
11220	1\\
11250	1\\
11280	1\\
11310	1\\
11340	1\\
11370	1\\
11400	1\\
11430	1\\
11460	1\\
11490	1\\
11520	1\\
11550	1\\
11580	1\\
11610	1\\
11640	1\\
11670	1\\
11700	1\\
11730	1\\
11760	1\\
11790	1\\
11820	1\\
11850	1\\
11880	1\\
11910	1\\
11940	1\\
11970	1\\
12000	1\\
12030	1\\
12060	1\\
12090	1\\
12120	1\\
12150	1\\
12180	1\\
12210	1\\
12240	1\\
12270	1\\
12300	1\\
12330	1\\
12360	1\\
12390	1\\
12420	1\\
12450	1\\
12480	1\\
12510	1\\
12540	1\\
12570	1\\
12600	1\\
12630	1\\
12660	1\\
12690	1\\
12720	1\\
12750	1\\
12780	1\\
12810	1\\
12840	1\\
12870	1\\
12900	1\\
12930	1\\
12960	1\\
12990	1\\
13020	1\\
13050	1\\
13080	1\\
13110	1\\
13140	1\\
13170	1\\
13200	1\\
13230	1\\
13260	1\\
13290	1\\
13320	1\\
13350	1\\
13380	1\\
13410	1\\
13440	1\\
13470	1\\
13500	1\\
13530	1\\
13560	1\\
13590	1\\
13620	1\\
13650	1\\
13680	1\\
13710	1\\
13740	1\\
13770	1\\
13800	1\\
13830	1\\
13860	1\\
13890	1\\
13920	1\\
13950	1\\
13980	1\\
14010	1\\
14040	1\\
14070	1\\
14100	1\\
14130	1\\
14160	1\\
14190	1\\
14220	1\\
14250	1\\
14280	1\\
14310	1\\
14340	1\\
14370	1\\
14400	1\\
14430	1\\
14460	1\\
14490	1\\
14520	1\\
14550	1\\
14580	1\\
14610	1\\
14640	1\\
14670	1\\
14700	1\\
14730	1\\
14760	1\\
14790	1\\
14820	1\\
14850	1\\
14880	1\\
14910	1\\
14940	1\\
14970	1\\
15000	1\\
15030	1\\
15060	1\\
15090	1\\
15120	1\\
15150	1\\
15180	1\\
15210	1\\
15240	1\\
15270	1\\
15300	1\\
};
\addlegendentry{\small Proposed method}

\addplot [color=mycolor1, dashed, mark repeat=1, line width=1.0pt, mark=none, mark options={mark size=2pt,solid, line width=0.5pt}]
  table[row sep=crcr]{%
0	0.0130914825812426\\
10	0.0222093448859156\\
20	0.0342086471992527\\
30	0.0485522159026703\\
40	0.0662598166186512\\
50	0.0859656603403892\\
60	0.108776280753473\\
70	0.133771985276024\\
80	0.1602301768488\\
90	0.190117967752106\\
100	0.221680781862375\\
110	0.239025463477443\\
120	0.25693833952061\\
130	0.27511895954836\\
140	0.294425035355589\\
150	0.31493646332161\\
160	0.33487237114088\\
170	0.356320084983536\\
180	0.377631235040398\\
190	0.398850661823004\\
200	0.421240684023834\\
210	0.435220967877728\\
220	0.449925413201376\\
230	0.463318678659501\\
240	0.477364697065728\\
250	0.49220740193948\\
260	0.506161356958128\\
270	0.520390800851292\\
280	0.535276009118471\\
290	0.550479748006403\\
300	0.565440055967865\\
310	0.575346734389236\\
320	0.584862996486218\\
330	0.594775153123891\\
340	0.604102813411529\\
350	0.61346666067608\\
360	0.623092315493506\\
370	0.633422566276581\\
380	0.643442543337838\\
390	0.653517068554265\\
400	0.663723259247131\\
410	0.670519950671445\\
420	0.67733905872554\\
430	0.684238447304727\\
440	0.691149008099567\\
450	0.69800291134684\\
460	0.705143412186459\\
470	0.712083349459971\\
480	0.719368217691837\\
490	0.726255132065177\\
500	0.733530547396923\\
510	0.738534635455249\\
520	0.743205070100913\\
530	0.748234166782091\\
540	0.75322365747348\\
550	0.758637598334459\\
560	0.763344398018668\\
570	0.768501625829696\\
580	0.773337418426234\\
590	0.778241818492654\\
600	0.783273289553506\\
610	0.786973407145853\\
620	0.790512591829201\\
630	0.794510838616271\\
640	0.798262422948176\\
650	0.802042741786395\\
660	0.805899304731188\\
670	0.809570827305842\\
680	0.81345545076382\\
690	0.817142969776709\\
700	0.820720982970003\\
710	0.823423497055912\\
720	0.826379577210155\\
730	0.829420721557202\\
740	0.832432740113154\\
750	0.835276305076611\\
760	0.838324851211549\\
770	0.841275950830186\\
780	0.844260411126536\\
790	0.847266988179287\\
800	0.850284190116245\\
810	0.852510824785977\\
820	0.854650756245564\\
830	0.856751080617587\\
840	0.859131273140557\\
850	0.861387107261832\\
860	0.863616812495226\\
870	0.865802323666436\\
880	0.868274170914233\\
890	0.870441900121007\\
900	0.872819964448118\\
910	0.874483499281305\\
920	0.876293977371064\\
930	0.878033270297896\\
940	0.879677150014788\\
950	0.88142803355044\\
960	0.883096834676252\\
970	0.884757144739203\\
980	0.8866848397958\\
990	0.888538811394777\\
1000	0.89041973976722\\
1010	0.891935525108928\\
1020	0.89318437539283\\
1030	0.894739753910326\\
1040	0.89625523838452\\
1050	0.897566500423012\\
1060	0.899045602157866\\
1070	0.900418349566461\\
1080	0.901677455617032\\
1090	0.902994139736602\\
1100	0.904460881692605\\
1110	0.905707785099916\\
1120	0.906841740892414\\
1130	0.907911112231001\\
1140	0.90899271668238\\
1150	0.910217938723993\\
1160	0.911400725386523\\
1170	0.912685566978849\\
1180	0.913919785625394\\
1190	0.915022095429925\\
1200	0.916144615751732\\
1210	0.917261620350438\\
1220	0.918252541356409\\
1230	0.919255111090436\\
1240	0.920251855284927\\
1250	0.921260302601759\\
1260	0.922173329223277\\
1270	0.923193631956915\\
1280	0.924328393803867\\
1290	0.925348825494538\\
1300	0.926271831957194\\
1310	0.927007864320527\\
1320	0.927796435676737\\
1330	0.928624927305757\\
1340	0.929356277251356\\
1350	0.930242989578567\\
1360	0.931020958554268\\
1370	0.931774323427546\\
1380	0.932563373692006\\
1390	0.933374810948045\\
1400	0.934214435182574\\
1410	0.9348637131398\\
1420	0.935585212922383\\
1430	0.936275748810762\\
1440	0.936978095202467\\
1450	0.937809940374399\\
1460	0.938567276343158\\
1470	0.939319020875926\\
1480	0.940005881062812\\
1490	0.940729208551547\\
1500	0.941383079049934\\
1510	0.941901669079143\\
1520	0.942447630512193\\
1530	0.943123775934036\\
1540	0.943740443886332\\
1550	0.944247400239272\\
1560	0.944862673515097\\
1570	0.945435163033824\\
1580	0.946041112243926\\
1590	0.946675139628814\\
1600	0.947241506670568\\
1610	0.947704654648212\\
1620	0.948316176522158\\
1630	0.948809446543329\\
1640	0.949299916589231\\
1650	0.949768949000738\\
1660	0.950370258213717\\
1670	0.950845733142763\\
1680	0.951344054995373\\
1690	0.951788962448077\\
1700	0.952280664613601\\
1710	0.952750683629118\\
1720	0.953129775547929\\
1730	0.953545753673705\\
1740	0.9540402394124\\
1750	0.954530806556414\\
1760	0.954997398659673\\
1770	0.955432129083877\\
1780	0.955831281110122\\
1790	0.95621213952785\\
1800	0.956600500078693\\
1810	0.956965561871452\\
1820	0.957296268678914\\
1830	0.957678678701409\\
1840	0.958062593908267\\
1850	0.958419318664265\\
1860	0.958795574511862\\
1870	0.959159115258631\\
1880	0.959529446403901\\
1890	0.959890685736692\\
1900	0.960249916118414\\
1910	0.960592683800026\\
1920	0.960909980470429\\
1930	0.961219076742826\\
1940	0.961567962048722\\
1950	0.961924867136528\\
1960	0.962263362964882\\
1970	0.962622000287176\\
1980	0.962954972569456\\
1990	0.963311664283286\\
2000	0.96364220621502\\
2010	0.963891217382592\\
2020	0.964202560197218\\
2030	0.964486675467672\\
2040	0.964781188278531\\
2050	0.965121550143149\\
2060	0.965443539812591\\
2070	0.96573169396066\\
2080	0.9660072905544\\
2090	0.96631129897012\\
2100	0.966587660298189\\
2110	0.966854392611935\\
2120	0.967113927003778\\
2130	0.967348153100909\\
2140	0.96758178744558\\
2150	0.967859277166153\\
2160	0.968145757274046\\
2170	0.968380679153838\\
2180	0.968689491357828\\
2190	0.96896970370609\\
2200	0.969245606139074\\
2210	0.969527304412341\\
2220	0.969733098523778\\
2230	0.969923568822935\\
2240	0.97015471838446\\
2250	0.970377755670311\\
2260	0.970590735344238\\
2270	0.970818334055602\\
2280	0.971041057199701\\
2290	0.971293875011842\\
2300	0.971498435470086\\
2310	0.971701861519905\\
2320	0.971949855757319\\
2330	0.972154121950225\\
2340	0.972355274140738\\
2350	0.972553056757338\\
2360	0.972762776424141\\
2370	0.972987413004018\\
2380	0.973182956158457\\
2390	0.973420492025702\\
2400	0.973647004048878\\
2410	0.973872447637891\\
2420	0.974069099626559\\
2430	0.974259596951648\\
2440	0.974401301084372\\
2450	0.974570200303071\\
2460	0.974786064482762\\
2470	0.974963885131223\\
2480	0.975144993222482\\
2490	0.975318950186277\\
2500	0.975480412365903\\
2510	0.975657738074803\\
2520	0.975829566297451\\
2530	0.976035030812152\\
2540	0.97619699988438\\
2550	0.976341141744198\\
2560	0.976499428706964\\
2570	0.976652582512695\\
2580	0.976823069437528\\
2590	0.976967989673856\\
2600	0.977132713706956\\
2610	0.977267737340591\\
2620	0.977425419372291\\
2630	0.977562363419911\\
2640	0.97771533125903\\
2650	0.977870578011774\\
2660	0.978009881670177\\
2670	0.978157580173218\\
2680	0.978295269464365\\
2690	0.978452990608779\\
2700	0.978615631151099\\
2710	0.978745182061047\\
2720	0.978839698690741\\
2730	0.978993273430877\\
2740	0.979138031111779\\
2750	0.979257431747864\\
2760	0.979387875131679\\
2770	0.979514665096221\\
2780	0.979652117627666\\
2790	0.979777687251061\\
2800	0.979906971813866\\
2810	0.98001091206185\\
2820	0.980155369271164\\
2830	0.980275390840951\\
2840	0.98038660335995\\
2850	0.980514106227767\\
2860	0.980653070582918\\
2870	0.980780915928166\\
2880	0.980927958884582\\
2890	0.981056929315337\\
2900	0.9811709965462\\
2910	0.981269013123695\\
2920	0.981393973834359\\
2930	0.981505631759775\\
2940	0.981609597069181\\
2950	0.981735003511279\\
2960	0.98184733593532\\
2970	0.981942610523553\\
2980	0.982056010361006\\
2990	0.982190547694882\\
3000	0.982304875358356\\
3010	0.98240747815877\\
3020	0.982508721744304\\
3030	0.982617159800723\\
3040	0.98271464539486\\
3050	0.982809723443558\\
3060	0.982911824489136\\
3070	0.9830065982046\\
3080	0.98311861097946\\
3090	0.983243206434272\\
3100	0.983341867808398\\
3110	0.98343533358054\\
3120	0.983531289515697\\
3130	0.983647756311169\\
3140	0.983765913051673\\
3150	0.98384691826197\\
3160	0.983925524881727\\
3170	0.984004153484401\\
3180	0.98408563125777\\
3190	0.984183884104802\\
3200	0.98426821835032\\
3210	0.98434640587909\\
3220	0.984419544984793\\
3230	0.98451077998345\\
3240	0.984610287225256\\
3250	0.984697031877671\\
3260	0.984771908883293\\
3270	0.984850060692681\\
3280	0.984937686330824\\
3290	0.985033657989864\\
3300	0.985100258640405\\
3310	0.985176803053854\\
3320	0.985264223784252\\
3330	0.985350289158027\\
3340	0.985423485068268\\
3350	0.985507746399769\\
3360	0.985581643739197\\
3370	0.985654661916053\\
3380	0.985738443015706\\
3390	0.985815665842672\\
3400	0.985905589095864\\
3410	0.985980070190675\\
3420	0.986046456863318\\
3430	0.986119555574248\\
3440	0.986177649655232\\
3450	0.986256484154847\\
3460	0.986329609528764\\
3470	0.986392476893468\\
3480	0.986460348731309\\
3490	0.986547101562874\\
3500	0.986622043733383\\
3510	0.98669589551306\\
3520	0.986752987356523\\
3530	0.986817780003666\\
3540	0.986881340320993\\
3550	0.986946024162463\\
3560	0.987004320855904\\
3570	0.987088463985021\\
3580	0.9871498059332\\
3590	0.987209627498687\\
3600	0.987273781471669\\
3610	0.987341551787084\\
3620	0.987403578145096\\
3630	0.987474993411319\\
3640	0.987530559517112\\
3650	0.987603398734976\\
3660	0.987670310534958\\
3670	0.987737544424791\\
3680	0.987806464677022\\
3690	0.987869038608908\\
3700	0.987919393229505\\
3710	0.987978078590951\\
3720	0.988023105290981\\
3730	0.988086359312107\\
3740	0.988133693269173\\
3750	0.988185268449692\\
3760	0.988253607695059\\
3770	0.988331610744269\\
3780	0.988391431637843\\
3790	0.988450726587066\\
3800	0.988501321088135\\
3810	0.988554805748165\\
3820	0.988599982689484\\
3830	0.988639550944468\\
3840	0.98868287395961\\
3850	0.988743300655492\\
3860	0.988793754940885\\
3870	0.988843390684017\\
3880	0.988892562404777\\
3890	0.988940484709238\\
3900	0.988992008691088\\
3910	0.989038686091952\\
3920	0.989098655475126\\
3930	0.98914755529833\\
3940	0.989195029338872\\
3950	0.989246570000158\\
3960	0.989285711926762\\
3970	0.989349348852238\\
3980	0.989400380066168\\
3990	0.989452278303844\\
4000	0.989497099543483\\
4010	0.989540111659521\\
4020	0.989591956270114\\
4030	0.989645029911122\\
4040	0.989682869942191\\
4050	0.989731476649452\\
4060	0.989780558847024\\
4070	0.989817882804287\\
4080	0.989874098293715\\
4090	0.989919840678891\\
4100	0.989972606198228\\
4110	0.990014159405195\\
4120	0.990055567252962\\
4130	0.990091955110294\\
4140	0.990142550960025\\
4150	0.990192787892078\\
4160	0.990226480939795\\
4170	0.990263884264276\\
4180	0.990301637714874\\
4190	0.990341618491987\\
4200	0.990396400456521\\
4210	0.990437709944713\\
4220	0.99048560675413\\
4230	0.990522559015602\\
4240	0.990566998917826\\
4250	0.990610887223049\\
4260	0.99065556672114\\
4270	0.990701070513721\\
4280	0.990739744068294\\
4290	0.990779230731759\\
4300	0.990827837680472\\
4310	0.990865187721018\\
4320	0.990899437510352\\
4330	0.990941556771608\\
4340	0.990976288776448\\
4350	0.99101291965061\\
4360	0.991044589079109\\
4370	0.991076513005091\\
4380	0.991111441224499\\
4390	0.991141100579166\\
4400	0.991180405163253\\
4410	0.991218120785654\\
4420	0.991252073946808\\
4430	0.991289180129597\\
4440	0.991329929971066\\
4450	0.991363349924927\\
4460	0.991404103241738\\
4470	0.991440004505659\\
4480	0.991487429107973\\
4490	0.991520214054271\\
4500	0.991556413432442\\
4510	0.991585328833392\\
4520	0.991624139775628\\
4530	0.991654036819874\\
4540	0.991691423748681\\
4550	0.991732023013839\\
4560	0.991760789564841\\
4570	0.991801596615423\\
4580	0.991836644726798\\
4590	0.991865479369522\\
4600	0.991905444450321\\
4610	0.991940311159926\\
4620	0.99197277076228\\
4630	0.992000781326872\\
4640	0.992028117680355\\
4650	0.992057365323655\\
4660	0.992095678451945\\
4670	0.992136573167932\\
4680	0.992167165250336\\
4690	0.992198020185435\\
4700	0.992225507704925\\
4710	0.992263036631404\\
4720	0.992297265378602\\
4730	0.992327172305855\\
4740	0.992360438035846\\
4750	0.992390071877314\\
4760	0.992413785327715\\
4770	0.992448204979132\\
4780	0.992471233948501\\
4790	0.992503516397414\\
4800	0.992537453497304\\
4810	0.992558150880926\\
4820	0.992582802380645\\
4830	0.992606499695442\\
4840	0.992631666442464\\
4850	0.992660928835251\\
4860	0.99268764843677\\
4870	0.992717389851571\\
4880	0.992741750024878\\
4890	0.992767169800022\\
4900	0.99278582093833\\
4910	0.992815078956845\\
4920	0.992843878954982\\
4930	0.992867757178103\\
4940	0.992898451318494\\
4950	0.992929155618119\\
4960	0.9929613920195\\
4970	0.99299347610884\\
4980	0.993022156344299\\
4990	0.993049366770054\\
5000	0.993079235887139\\
5010	0.993099814505485\\
5020	0.993126759976065\\
5030	0.993150073462751\\
5040	0.993172016231721\\
5050	0.993198511388396\\
5060	0.99322292310776\\
5070	0.993247076531495\\
5080	0.99328231100866\\
5090	0.993299165598647\\
5100	0.993324534703962\\
};
\addlegendentry{\small Random method}
\end{axis}
\end{tikzpicture}%
